A note on information theoretic characterizations of physical theories

Clifton, Bub, and Halvorson [Foundations of Physics 33, 1561 (2003)] have recently argued that quantum theory is characterized by its satisfaction of three information-theoretic axioms. However, it is not difficult to construct apparent counterexamples to the CBH characterization theorem. In this paper, we discuss the limits of the characterization theorem, and we provide some technical tools for checking whether a theory (specified in terms of the convex structure of its state space) falls within these limits.

==> pst-3dplot.tex <==
%%
%% This is file `pst-3dplot.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-3dplot.tex'
%%
%% Herbert Voss <voss@perce.de>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-3dplot' is a PSTricks package to draw 3d curves and graphical objects
%%
\def\fileversion{1.2b}
\def\filedate{2003/11/03}
\message{`PST-3dplot' v\fileversion, \filedate\space (Herbert Voss)}
\csname PSTThreeDplotLoaded\endcsname
\let\PSTThreeDplotLoaded\endinput
% Requires PSTricks, pst-node, pst-plot, multido packages
%\usepackage{pstcol}
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
\ifx\PSTplotLoaded\endinput\else\input pst-plot.tex\fi% plotpoints
\ifx\PSTNewThreeDLoaded\endinput\else\input pst-vue3d.tex\fi
\ifx\PSTMultidoLoaded\endinput\else\input multido.tex\fi
%
% DPC interface to the `keyval' package (until keyval based version of PSTricks)
\input pst-key
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor
%
%%%%%%%%%%%%%%%%%% Macrolist %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \def\variablesThreeD
% \def\pstThreeDPut
% \def\pstThreeDLine
% \def\pstThreeDDot
% \def\pstThreeDNode
% \def\pstUThreeDPut
% \def\pstThreeDSquare
% \def\pstThreeDBox
% \def\pstThreeDSphere
% \def\pstThreeDEllipse
% \def\pstThreeDPlotFunc
% \def\psplotThreeD
% \def\parametricplotThreeD
% \def\psThreeDPlot
% \def\pstThreeDCoor
% \def\fileplotThreeD
% \def\dataplotThreeD
% \def\listplotThreeD
%
%
\newdimen\pst@dimf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ---------------- the if's -----------------
%
\newif\ifPst@drawing%			draw the coordinates?
\define@key{psset}{drawing}[true]{%
	\@nameuse{Pst@drawing#1}%
}
\newif\ifPst@drawCoor%		draw the coordinates of a dot?
\define@key{psset}{drawCoor}[false]{%
	\@nameuse{Pst@drawCoor#1}%
}
\newif\ifPst@hiddenLine%	emulate hidden line surface?
\define@key{psset}{hiddenLine}[false]{%
	\@nameuse{Pst@hiddenLine#1}%
}
%
% ------- the global definitions for the pspicture frame ------
%
\define@key{psset}{xMin}{\edef\psk@ThreeDplot@xMin{#1}}
\define@key{psset}{xMax}{\edef\psk@ThreeDplot@xMax{#1}}
\define@key{psset}{yMin}{\edef\psk@ThreeDplot@yMin{#1}}
\define@key{psset}{yMax}{\edef\psk@ThreeDplot@yMax{#1}}
\define@key{psset}{zMin}{\edef\psk@ThreeDplot@zMin{#1}}
\define@key{psset}{zMax}{\edef\psk@ThreeDplot@zMax{#1}}
\define@key{psset}{xThreeDunit}{\edef\psk@ThreeDplot@xThreeDunit{#1}}
\define@key{psset}{yThreeDunit}{\edef\psk@ThreeDplot@yThreeDunit{#1}}
\define@key{psset}{zThreeDunit}{\edef\psk@ThreeDplot@zThreeDunit{#1}}
%
% -------------- the angles and the plotpoints -------------
%
\define@key{psset}{Alpha}{%			Horizontal turn
	\edef\psk@ThreeDplot@Alpha{#1}%
}
\define@key{psset}{Beta}{%			Vertical turn
	\edef\psk@ThreeDplot@Beta{#1}%
}
\define@key{psset}{drawStyle}{%			how to draw 3D functions
	\edef\psk@ThreeDplot@drawStyle{#1}%
}
\def\drawStyle@xLines{xLines}
\def\drawStyle@yLines{yLines}
\def\drawStyle@xyLines{xyLines}
\def\drawStyle@yxLines{yxLines}
%
\define@key{psset}{xPlotpoints}{%		points in x direction
	\edef\psk@ThreeDplot@xPlotpoints{#1}%
}
\define@key{psset}{yPlotpoints}{%		points in y direction
	\edef\psk@ThreeDplot@yPlotpoints{#1}%
}
\define@key{psset}{beginAngle}{%		for ellipse/circle arc
	\edef\psk@ThreeDplot@beginAngle{#1}%
}
\define@key{psset}{endAngle}{%			for ellipse/circle arc
	\edef\psk@ThreeDplot@endAngle{#1}%
}
\define@key{psset}{linejoin}{%		how lines come together 0,1,2
	\edef\psk@ThreeDplot@linejoin{#1}%
}
\define@key{psset}{plane}{%			xy,xz,yz
	\edef\psk@ThreeDplot@plane{#1}%
}
\define@key{psset}{origin}{%			combination of (lr)(tBb)
	\edef\psk@ThreeDplot@origin{#1}%
}
\def\ThreeDplot@planeXY{xy}
\def\ThreeDplot@planeXZ{xz}
\def\ThreeDplot@planeYZ{yz}
%
% -------------- the length and node definitions -------------
%
\define@key{psset}{XO}{%			the X-offset
	\edef\psk@ThreeDplot@XO{#1}%
}
\define@key{psset}{YO}{%			the y-offset
	\edef\psk@ThreeDplot@YO{#1}%
}
\define@key{psset}{angleStep}{%		for circles
	\edef\psk@ThreeDplot@angleStep{#1}%
}
\define@key{psset}{posStart}{%		where the arrows start
	\edef\psk@ThreeDplot@posStart{#1}%
}
\define@key{psset}{length}{%		the length of the before|outlines
	\edef\psk@ThreeDplot@length{#1}%
}
\define@key{psset}{arrowOffset}{%	offset for \arrowLine
	\edef\psk@ThreeDplot@arrowOffset{#1}%
}
\define@key{psset}{visibleLineStyle}{%	offset for \arrowLine
	\edef\psk@ThreeDplot@visibleLineStyle{#1}%
}
\define@key{psset}{invisibleLineStyle}{%	offset for \arrowLine
	\edef\psk@ThreeDplot@invisibleLineStyle{#1}%
}
%
\define@key{psset}{nameX}{%		start of the object arrow
	\edef\psk@ThreeDplot@nameX{#1}%
}
\define@key{psset}{spotX}{%		where to draw the label
	\edef\psk@ThreeDplot@spotX{#1}%
}
\define@key{psset}{nameY}{%
	\edef\psk@ThreeDplot@nameY{#1}%
}
\define@key{psset}{spotY}{%
	\edef\psk@ThreeDplot@spotY{#1}%
}
\define@key{psset}{nameZ}{%
	\edef\psk@ThreeDplot@nameZ{#1}%
}
\define@key{psset}{spotZ}{%
	\edef\psk@ThreeDplot@spotZ{#1}%
}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                              %
%                        B A S I C S	                       %
%                                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\setDefaults{%
    \setkeys{psset}{%
	drawing=true,hiddenLine=false,%
	xMin=-1,xMax=4,yMin=-1,yMax=4,zMin=-1,zMax=4,%
	xThreeDunit=1,yThreeDunit=1,zThreeDunit=1,%
	Alpha=45,Beta=30,%
	drawStyle=xLines,%
	xPlotpoints=25,yPlotpoints=25,%
	beginAngle=0,endAngle=360,%
	linejoin=1,%
	XO=0,YO=0,%
	angleStep=1,%
	posStart=0,length=2,%
	arrowOffset=0,%
	visibleLineStyle=solid,%
	invisibleLineStyle=dashed,%
	nameX=x,spotX=180,%
	nameY=y,spotY=0,%
	nameZ=z,spotZ=90,%
	plane=xy,origin=c%
    }%
}
\setDefaults
%
% (#1) -> #1 #2 #3
%
\def\getThreeDCoor#1#2{\pst@getThreeDcoor(#1)\let#2\pst@coorIIID}
\def\pst@getThreeDcoor(#1,#2,#3){%
	\edef\pst@coorIIID{#1\space #2\space #3\space}
}
\def\variablesThreeD{%
	/Alpha \psk@ThreeDplot@Alpha\space def
	/Beta \psk@ThreeDplot@Beta\space def
	/Convert {			% now we have x y z
		3 -1 roll		% y z x
		dup			% y z x x
		neg Alpha cos mul	% y z x (x)
		4 -1 roll		% z x (x) y
		dup			% z x (x) y y
		5 1 roll		% y z x (x) y
		Alpha sin mul add 	% y z x (x2)
		4 1 roll		% (x2) y z x
		Alpha sin mul		% (x2) y z (x)
		3 -1 roll		% (x2) z (x) y
		Alpha cos mul add neg Beta sin mul % (x2) z (x)
		exch			% (x2) (x) z
		Beta cos mul add 	% (x2) (y2)
	} def
	\pst@tempa\space Convert
	/y2DA exch def
	/x2DA exch def
	\pst@tempb\space Convert
	/y2DB exch def
	/x2DB exch def
	\pst@tempc\space Convert
	/y2DC exch def
	/x2DC exch def
}
\def\pst@addThreeDVec(#1)(#2)#3#4#5{%
	\pst@calcThreeDVec(#1)(#2)%
	\let#3\pst@getValueX%
	\let#4\pst@getValueY%
	\let#5\pst@getValueZ%
}
\def\pst@subThreeDVec(#1)(#2,#3,#4)#5#6#7{%
	\pst@calcThreeDVec(#1)(-#2,-#3,-#4)%
	\let#5\pst@getValueX%
	\let#6\pst@getValueY%
	\let#7\pst@getValueZ%
}
\def\pst@calcThreeDVec(#1,#2,#3)(#4,#5,#6){%
  \begingroup
    \pst@dima=#1 pt%
    \pst@dimb=#2 pt%
    \pst@dimc=#3 pt%
	\pst@dimf=#4 pt%
	\pst@dimg=#5 pt%
	\pst@dimh=#6 pt%
	\advance\pst@dima by \pst@dimf%
	\advance\pst@dimb by \pst@dimg%
	\advance\pst@dimc by \pst@dimh%
	\xdef\pst@getValueX{\pst@number\pst@dima}%
	\xdef\pst@getValueY{\pst@number\pst@dimb}%
	\xdef\pst@getValueZ{\pst@number\pst@dimc}%
  \endgroup
}%
%
% the ThreeD coordinate system
%
\def\pstThreeDCoor{\@ifnextchar[{\pst@ThreeDCoor}{\pst@ThreeDCoor[]}}
\def\pst@ThreeDCoor[#1]{{%
	\pst@killglue
	\setkeys{psset}{linewidth=0.5pt,linecolor=red,arrows=->,dotstyle=|}
	\setkeys{psset}{#1}
	\pstThreeDNode(\psk@ThreeDplot@xMin,0,0){xMin}
	\pstThreeDNode(\psk@ThreeDplot@xMax,0,0){xMax}
	\pstThreeDNode(0,\psk@ThreeDplot@yMin,0){yMin}
	\pstThreeDNode(0,\psk@ThreeDplot@yMax,0){yMax}
	\pstThreeDNode(0,0,\psk@ThreeDplot@zMin){zMin}
	\pstThreeDNode(0,0,\psk@ThreeDplot@zMax){zMax}
	\ifPst@drawing
	    % ThreeDplot axes
	    \psline(xMin)(xMax)
	    \psline(yMin)(yMax)
	    \psline(zMin)(zMax)
	    \uput[\psk@ThreeDplot@spotX](xMax){$\mathbf{\psk@ThreeDplot@nameX}$}
	    \uput[\psk@ThreeDplot@spotY](yMax){$\mathbf{\psk@ThreeDplot@nameY}$}
	    \uput[\psk@ThreeDplot@spotZ](zMax){$\mathbf{\psk@ThreeDplot@nameZ}$}
	\fi% ifdrawing
}}
%
% put anything at (#2,#3,#4)
%
\def\pstThreeDPut{\@ifnextchar[{\pst@ThreeDPut}{\pst@ThreeDPut[]}}
\def\pst@ThreeDPut[#1](#2,#3,#4)#5{{%
	\pst@killglue%
	\setkeys{psset}{#1}
	\pstThreeDNode(#2,#3,#4){temp@pstNode}%
%	\def\@tempa{c}
%	\ifx\pst@ThreeDplot@origin\@tempa%
%	    \rput(temp@pstNode){#5}%
%	\else%
	    \rput[\psk@ThreeDplot@origin](temp@pstNode){#5}%
%	\fi%
}}
%
% draws a 3d line
%
\def\pstThreeDLine{\@ifnextchar[{\pst@ThreeDLine}{\pst@ThreeDLine[]}}
\def\pst@ThreeDLine[#1](#2,#3,#4)(#5,#6,#7){{%
	\pst@killglue
	\setkeys{psset}{#1}
	\def\pst@ThreeDplot@x{#2}	% x coordinate
	\def\pst@ThreeDplot@y{#3}	% y coordinate
	\def\pst@ThreeDplot@z{#4}	% z coordinate
	\def\pst@ThreeDplot@xB{#5}	% x coordinate
	\def\pst@ThreeDplot@yB{#6}	% y coordinate
	\def\pst@ThreeDplot@zB{#7}	% z coordinate
	\psline(!%
%		/Alpha \psk@ThreeDplot@Alpha\space def
%		/Beta \psk@ThreeDplot@Beta\space def
		/x \pst@ThreeDplot@x\space def
		/y \pst@ThreeDplot@y\space def
		/z \pst@ThreeDplot@z\space def
		/x2D x neg Alpha cos mul y Alpha sin mul add def
		/y2D x Alpha sin mul y Alpha cos mul add neg Beta sin mul
			z Beta cos mul add def
		x2D y2D)(!%
		/xB \pst@ThreeDplot@xB\space def
		/yB \pst@ThreeDplot@yB\space def
		/zB \pst@ThreeDplot@zB\space def
		/x2DB xB neg Alpha cos mul yB Alpha sin mul add def
		/y2DB xB Alpha sin mul yB Alpha cos mul add neg Beta sin mul
			zB Beta cos mul add def
		x2DB y2DB)
}}
%
% set a 3d dot
%
\def\pstThreeDDot{\@ifnextchar[{\pst@ThreeDDot}{\pst@ThreeDDot[]}}
\def\pst@ThreeDDot[#1](#2,#3,#4){{%
%	\pst@killglue
	\setkeys{psset}{linestyle=dashed,linewidth=0.5pt}% default
	\setkeys{psset}{#1}
	\pstThreeDNode(#2,#3,#4){A}
	\psdots(A)
	\ifPst@drawCoor
		\pstThreeDNode(#2,#3,0){B}
		\psline[#1](A)(B)
		\pstThreeDNode(#2,0,0){A}
		\psline[#1](B)(A)
		\pstThreeDNode(0,#3,0){A}
		\psline[#1](B)(A)
	\fi
}}
%
% transform the 3d coordinates of the node (#1,#2,#3)
% into a 2d node with the name #4
%
\def\pstThreeDNode(#1,#2,#3)#4{%
	\def\pst@ThreeDplot@x{#1}	% x coordinate
	\def\pst@ThreeDplot@y{#2}	% y coordinate
	\def\pst@ThreeDplot@z{#3}	% z coordinate
	\pnode(!%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/x \pst@ThreeDplot@x\space def
		/y \pst@ThreeDplot@y\space def
		/z \pst@ThreeDplot@z\space def
		x neg Alpha cos mul y Alpha sin mul add 
		x Alpha sin mul y Alpha cos mul add neg Beta sin mul
		    z Beta cos mul add ){#4}%
}
%
% a 3d uput[](){}
%
\def\pstUThreeDPut{\@ifnextchar[{\pst@UThreeDPut}{\pst@UThreeDPut[]}}
\def\pst@UThreeDPut[#1](#2,#3,#4)#5{{%
	\def\pst@ThreeDplot@x{#2}	% x coordinate
	\def\pst@ThreeDplot@y{#3}	% y coordinate
	\def\pst@ThreeDplot@z{#4}	% z coordinate
	\uput[#1](!%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/x \pst@ThreeDplot@x\space def
		/y \pst@ThreeDplot@y\space def
		/z \pst@ThreeDplot@z\space def
		/x2D x neg Alpha cos mul y Alpha sin mul add def
		/y2D x Alpha sin mul y Alpha cos mul add neg Beta sin mul 
			z Beta cos mul add def
	 	x2D y2D){#5}
}}
%
% Trangle [options](Point1)(Point2)(Point3)
%
\def\pstThreeDTriangle{%
	\@ifnextchar[%
		{\do@ThreeDTriangle}%
		{\do@ThreeDTriangle[]}%
}
\def\do@ThreeDTriangle[#1](#2)(#3)(#4){{%
	\ifx#1\empty\else\setkeys{psset}{#1}\fi%
	\ifPst@drawCoor
		\pstThreeDDot[drawCoor=true](#2)%
		\pstThreeDDot[drawCoor=true](#3)%
		\pstThreeDDot[drawCoor=true](#4)%
	\fi
	\pstThreeDNode(#2){A}
	\pstThreeDNode(#3){B}
	\pstThreeDNode(#4){C}
	\def\@tempa{none}%
	\ifx\psk@fillstyle\@tempa
	\else
		\pscustom{%
			\code{\psk@ThreeDplot@linejoin\space setlinejoin}%
	\fi%
		\psline[#1](A)(B)(C)(A)
	\ifx\psk@fillstyle\@tempa\else}\fi%
}}
%
% draws a threeD square as a polygon 
%
% [#1] options
% (#2) starting vector ax,ay,az
% (#3) first direction vector ux,uy,uz
% (#4) second direction vector wx,wy,wz
%
\def\pstThreeDSquare{\@ifnextchar[{\doThreeDSquare}{\doThreeDSquare[]}}
\def\doThreeDSquare[#1](#2)(#3)(#4){{%
	\psset{#1}
	\getThreeDCoor{#2}\pst@tempa	% 1. point 
	\getThreeDCoor{#3}\pst@tempb	% 2. point
	\getThreeDCoor{#4}\pst@tempc	% 3. point
	\addto@pscode{%
		\variablesThreeD
	}% end code ps
	\psline(! x2DA y2DA)(! x2DA x2DB add y2DA y2DB add)% A -> B
		(! x2DA x2DB add x2DC add y2DA y2DB add y2DC add)%  -> C
		(! x2DA x2DC add y2DA y2DC add)%  -> D
		(! x2DA y2DA)% -> A
	\ifPst@drawCoor%
		{%
		\psset{linestyle=dashed,linewidth=0.5pt}%
		\pstThreeDDot(#2)%
		\pst@addThreeDVec(#2)(#3)\pst@tempa\pst@tempb\pst@tempc
		\pstThreeDDot(\pst@tempa,\pst@tempb,\pst@tempc)
		\pst@addThreeDVec(#2)(#4)\pst@tempa\pst@tempb\pst@tempc
		\pstThreeDDot(\pst@tempa,\pst@tempb,\pst@tempc)
		\pst@addThreeDVec(\pst@tempa,\pst@tempb,\pst@tempc)%
			(#3)\pst@tempa\pst@tempb\pst@tempc
		\pstThreeDDot(\pst@tempa,\pst@tempb,\pst@tempc)%
		}%
	\fi%
}}

%
% draws a threeD Box
% [#1] options
% (#2) first direction vector ux,uy,uz
% (#3) second direction vector vx,vy,vz
% (#4) third direction vector wx,wy,wz
%
\def\pstThreeDBox{\@ifnextchar[{\doThreeDBox}{\doThreeDBox[]}}
\def\doThreeDBox[#1](#2)(#3)(#4)(#5){{%
	\psset{#1}
	{%	
	\psset{linestyle=\psk@ThreeDplot@invisibleLineStyle}
	\pstThreeDSquare(#2)(#4)(#5)% 	lower square
	\pstThreeDSquare(#2)(#3)(#4)% 	back square
	}{%
	\psset{linestyle=\psk@ThreeDplot@visibleLineStyle}
	\pst@addThreeDVec(#2)(#4)\pst@tempa\pst@tempb\pst@tempc
	\pstThreeDSquare(\pst@tempa,\pst@tempb,\pst@tempc)(#3)(#5)% left square
	\pst@addThreeDVec(#2)(#3)\pst@tempa\pst@tempb\pst@tempc
	\pstThreeDSquare(\pst@tempa,\pst@tempb,\pst@tempc)(#4)(#5)% top square
	\pst@addThreeDVec(#2)(#5)\pst@tempa\pst@tempb\pst@tempc
	\pstThreeDSquare(\pst@tempa,\pst@tempb,\pst@tempc)(#3)(#4)% front square
	}%
}}
%
% Sphere
%
\def\pstThreeDSphere{\@ifnextchar[{\pst@ThreeDSphere}{\pst@ThreeDSphere[]}}
\def\pst@ThreeDSphere[#1](#2,#3,#4)#5{{%
	\psset{CX=0,CZ=0,CY=0,%
		THETA=\psk@ThreeDplot@Beta,PHI=\psk@ThreeDplot@Beta,%
		Dobs=10,Decran=10}
	\psset{#1}
	\pstThreeDNode(#2,#3,#4){SphereCenter}
	\rput(SphereCenter){\SphereThreeD{#5}}
}}
%
% set a 3d ellipse/circle
%
% #1 options
% #2 center cx,cy,cz
% #3 radius ax,ay,az
% #4 radius bx,by,bz
%
\def\pstThreeDEllipse{\@ifnextchar[{\doThreeDEllipse}{\doThreeDEllipse[]}}
\def\doThreeDEllipse[#1](#2)(#3)(#4){{%
	\psset{plotstyle=curve,xPlotpoints=\psk@plotpoints}
	\psset{#1}		
	\getThreeDCoor{#2}\pst@tempc%	 center 
	\getThreeDCoor{#3}\pst@tempa%	 a 
	\getThreeDCoor{#4}\pst@tempb%	 b 
	\parametricplotThreeD(\psk@ThreeDplot@beginAngle,\psk@ThreeDplot@endAngle){%
		\pst@tempc\space \pst@tempa\space \pst@tempb\space 
		9 -1 roll t cos 8 -1 roll neg mul add t sin 5 -1 roll mul add
		7 -1 roll t cos 7 -1 roll neg mul add t sin 5 -1 roll mul add
		5 -1 roll t cos 6 -1 roll neg mul add t sin 5 -1 roll mul add
	}
}}
%
\def\pstThreeDCircle{\pstThreeDEllipse}
\def\pstThreeDPlotFunc{\psplotThreeD}%	only for compatibility
%
\def\pstRotPoint{\@ifnextchar[{\pstRotPointi}{\pstRotPointi[]}}
\def\pstRotPointi[#1](#2,#3,#4)(#5,#6,#7)#8{{%
	\setkeys{psset}{#1}
	\def\pst@ThreeDplot@x{#2}	% x coordinate
	\def\pst@ThreeDplot@y{#3}	% y coordinate
	\def\pst@ThreeDplot@z{#4}	% z coordinate
	\def\pst@ThreeDplot@ThetaX{#5}	% rotating angle
	\def\pst@ThreeDplot@ThetaY{#6}	% rotating angle
	\def\pst@ThreeDplot@ThetaZ{#7}	% rotating angle
	\pnode(!%
		/x \pst@ThreeDplot@x\space def
		/y \pst@ThreeDplot@y\space def
		/z \pst@ThreeDplot@z\space def
% rotating on the z-Axes
		/Theta \pst@ThreeDplot@ThetaZ\space def
		/x0 x Theta cos mul y Theta sin mul sub def
		/y x Theta sin mul y Theta cos mul add def
		/x x0 def
% rotating on the y-Axes
		/Theta \pst@ThreeDplot@ThetaY\space def
		/x0 x Theta cos mul z Theta sin mul add def
		/z x neg Theta sin mul z Theta cos mul add def
		/x x0 def
% rotating on the x-Axes
		/Theta \pst@ThreeDplot@ThetaX\space def
		/y0 y Theta cos mul z Theta sin mul sub def
		/z y Theta sin mul z Theta cos mul add def
		/y y0 def
%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/x2D x neg Alpha cos mul y Alpha sin mul add def
		/y2D x Alpha sin mul y Alpha cos mul add neg Beta sin mul z Beta cos mul add def
		x2D y2D){#8}%
}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\psplotinit#1{\xdef\psplot@init{#1 }}
\def\psplot@init{}
%
\def\psplotThreeD{\@ifnextchar[{\ps@plotThreeD}{\ps@plotThreeD[]}}
\def\ps@plotThreeD[#1](#2,#3)(#4,#5)#6{%
    \setkeys{psset}{hiddenLine=false,drawStyle=xLines}% default
    \setkeys{psset}{#1}
    \ifx\psk@ThreeDplot@drawStyle\drawStyle@xyLines
	\doPlotThreeD@xLines(#2,#3)(#4,#5){#6}
	\doPlotThreeD@yLines(#2,#3)(#4,#5){#6}
    \else
	\ifx\psk@ThreeDplot@drawStyle\drawStyle@yxLines
	    \doPlotThreeD@yLines(#2,#3)(#4,#5){#6}
	    \doPlotThreeD@xLines(#2,#3)(#4,#5){#6}
	\else
	    \ifx\psk@ThreeDplot@drawStyle\drawStyle@xLines
		\doPlotThreeD@xLines(#2,#3)(#4,#5){#6}
	    \fi
	    \ifx\psk@ThreeDplot@drawStyle\drawStyle@yLines
		\doPlotThreeD@yLines(#2,#3)(#4,#5){#6}
	    \fi
	\fi
    \fi
}
\def\doPlotThreeD@xLines{%
	\def\pst@par{}
	\pst@object{psplotThreeD@xLines}%
}
\def\doPlotThreeD@yLines{%
	\def\pst@par{}
	\pst@object{psplotThreeD@yLines}%
}
\def\psplotThreeD@xLines@i(#1,#2)(#3,#4)#5{%
    \pst@killglue
    \begingroup
	\use@par%
	\@pstfalse
	\@nameuse{beginplot@\psplotstyle}%
	\gdef\psplot@init{}%
	\@nameuse{testqp@\psplotstyle}%
	\if@pst%	lines and dots
	    \addto@pscode{%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/xMin #1 def
		/x xMin def
		/x1 #2 def
		/y #3 def
		/y1 #4 def
		/dx x1 x sub \psk@ThreeDplot@xPlotpoints\space div def
		/dy y1 y sub \psk@ThreeDplot@yPlotpoints\space div def
		/func {#5} def
		/xyz {
		    x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
		    x Alpha sin mul y Alpha cos mul add neg Beta sin mul
			func Beta cos mul add \pst@number\psyunit mul} def
	    }%
	    \psplotThreeD@xLines@ii
	\else%	curves
	    \endgroup
	    \multido{\n@Y=0+1}{\psk@ThreeDplot@yPlotpoints}{%
		\ifPst@hiddenLine\pscustom[fillcolor=white,fillstyle=solid]{\fi
		    \@nameuse{beginplot@\psplotstyle}%
			\addto@pscode{%
			    /Alpha \psk@ThreeDplot@Alpha\space def
			    /Beta \psk@ThreeDplot@Beta\space def
			    /xMin #1 def
			    /x xMin def
			    /x1 #2 def
			    /dx x1 x sub \psk@ThreeDplot@xPlotpoints\space div def
			    /dy #4\space #3\space sub \psk@ThreeDplot@yPlotpoints\space div def
			    /y #3\space \n@Y\space dy mul add def
			    /func {#5} def
			    /xyz {
				x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
				x Alpha sin mul y Alpha cos mul add neg Beta sin mul
				    func Beta cos mul add \pst@number\psyunit mul} def
			}%
		    \psplotThreeD@xLines@iii%
		\ifPst@hiddenLine }\fi%
	    }%
	\fi
    \endgroup
    \ignorespaces%
}
\def\psplotThreeD@xLines@ii{%
    \addto@pscode{%
	xyz \@nameuse{beginqp@\psplotstyle}
	\psk@ThreeDplot@yPlotpoints\space 1 add {
	    /x xMin def
	    xyz moveto
	    \psk@ThreeDplot@xPlotpoints\space 1 add {
		xyz \@nameuse{doqp@\psplotstyle}
		/x x dx add def
	    } repeat
	    /y y dy add def
	} repeat
	/x x1 def
	/y y1 def
	xyz \@nameuse{doqp@\psplotstyle}
    }%
    \@nameuse{endqp@\psplotstyle}%
}
\def\psplotThreeD@xLines@iii{%    curves
    \addto@pscode{%
	    /x xMin def
	    mark
	    /n 2 def
		\psk@ThreeDplot@xPlotpoints {
	    	    xyz
    		    n 2 roll
    		    /n n 2 add def
    		    /x x dx add def
    		} repeat
        /x x1 def
        xyz
        n 2 roll
    }%
    \@nameuse{endplot@\psplotstyle}%
}
%
\def\psplotThreeD@yLines@i(#1,#2)(#3,#4)#5{%
    \pst@killglue
    \begingroup
	\use@par%
	\@pstfalse
	\@nameuse{beginplot@\psplotstyle}%
	\gdef\psplot@init{}%
	\@nameuse{testqp@\psplotstyle}%
	\if@pst%	lines and dots
	    \addto@pscode{%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
    		/x #1 def
		/x1 #2 def
		/yMin #3 def
		/y yMin def
		/y1 #4 def
		/dx x1 x sub \psk@ThreeDplot@xPlotpoints\space div def
		/dy y1 y sub \psk@ThreeDplot@yPlotpoints\space div def
		/func {#5} def
		/xyz {
		    x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
		    x Alpha sin mul y Alpha cos mul add neg Beta sin mul
			func Beta cos mul add \pst@number\psyunit mul} def
	    }%
	    \psplotThreeD@yLines@ii
	\else%	curves
	    \endgroup
	    \multido{\n@X=0+1}{\psk@ThreeDplot@xPlotpoints}{%
		\ifPst@hiddenLine\pscustom[fillcolor=white,fillstyle=solid]{\fi
		    \@nameuse{beginplot@\psplotstyle}%
			\addto@pscode{%
			    /Alpha \psk@ThreeDplot@Alpha\space def
			    /Beta \psk@ThreeDplot@Beta\space def
			    /yMin #3 def
			    /y yMin def
			    /y1 #4 def
			    /dy y1 y sub \psk@ThreeDplot@yPlotpoints\space div def
			    /dx #2\space #1\space sub \psk@ThreeDplot@xPlotpoints\space div def
			    /x #1\space \n@X\space dx mul add def
			    /func {#5} def
			    /xyz {
				x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
				x Alpha sin mul y Alpha cos mul add neg Beta sin mul
				    func Beta cos mul add \pst@number\psyunit mul} def
			}%
		    \psplotThreeD@yLines@iii%
		\ifPst@hiddenLine }\fi%
	    }%
	\fi
    \endgroup
    \ignorespaces%
}
\def\psplotThreeD@yLines@ii{%
    \addto@pscode{%
	xyz \@nameuse{beginqp@\psplotstyle}
	\psk@ThreeDplot@xPlotpoints\space 1 add {
	    /y yMin def
	    xyz moveto
	    \psk@ThreeDplot@yPlotpoints\space 1 add {
		xyz \@nameuse{doqp@\psplotstyle}
		/y y dy add def
	    } repeat
	    /x x dx add def
	} repeat
	/x x1 def
	/y y1 def
	xyz \@nameuse{doqp@\psplotstyle}
    }%
    \@nameuse{endqp@\psplotstyle}%
}
\def\psplotThreeD@yLines@iii{%    curves
    \addto@pscode{%
	    /y yMin def
	    mark
	    /n 2 def
		\psk@ThreeDplot@yPlotpoints {
	    	    xyz
    		    n 2 roll
    		    /n n 2 add def
    		    /y y dy add def
    		} repeat
        /y y1 def
        xyz
        n 2 roll
    }%
    \@nameuse{endplot@\psplotstyle}%
}
%
% parametricplot ----------------------------------------------------------------
%
\def\parametricplotThreeD{%
	\@ifnextchar[%
		{\doParametricPlotThreeD}%
		{\doParametricPlotThreeD[]}%
}
\def\doParametricPlotThreeD[#1]{%
	\setkeys{psset}{#1}%
	\def\pst@par{}%
	\pst@object{psParamPlotThreeD}%
}
\def\psParamPlotThreeD@i(#1){%
	\@ifnextchar(%
		{\psParamPlotThreeD@ii(#1)}%
		{\psParamPlotThreeD@ii(#1)(0,0)}%
}
\def\psParamPlotThreeD@ii(#1,#2)(#3,#4)#5 {%
    \pst@killglue
    \begingroup
	\use@par%
	\@pstfalse
	\@nameuse{beginplot@\psplotstyle}%
	\gdef\parametricII@init{}%
	\@nameuse{testqp@\psplotstyle}%
	\if@pst
	    \addto@pscode{%
	    	/Alpha \psk@ThreeDplot@Alpha\space def
	    	/Beta \psk@ThreeDplot@Beta\space def
		/tMin #1 def
		/t tMin def
		/t1 #2 def
		/u #3 def
		/u1 #4 def
		/dt t1 t sub \psk@ThreeDplot@xPlotpoints\space div def
		/du u1 u sub \psk@ThreeDplot@yPlotpoints\space div def
		/xyz {
		    #5
		    3 -1 roll               % y z x
		    \psk@ThreeDplot@xThreeDunit\space div
		    dup                     % y z x x
		    neg Alpha cos mul       % y z x (x)
		    4 -1 roll               % z x (x) y
		    \psk@ThreeDplot@yThreeDunit\space div
		    dup                     % z x (x) y y
		    5 1 roll                % y z x (x) y
		    Alpha sin mul add \pst@number\psxunit mul       % y z x (x2)
		    4 1 roll                % (x2) y z x
		    Alpha sin mul           % (x2) y z (x)
		    3 -1 roll               % (x2) z (x) y
		    Alpha cos mul add neg Beta sin mul % (x2) z (x)
		    exch                    % (x2) (x) z
		    \psk@ThreeDplot@zThreeDunit\space div
		    Beta cos mul add \pst@number\psyunit mul        % (x2) (y2)
		} def
	    }%
	    \psParamPlotThreeD@iii%
	\else
	    \endgroup
	    \ifx#3#4\psset{yPlotpoints=1}\fi% do we have two different parameters or #3=#4
	    \multido{\n@Y=0+1}{\psk@ThreeDplot@yPlotpoints}{%
		\@nameuse{beginplot@\psplotstyle}%
		\addto@pscode{%
		    /Alpha \psk@ThreeDplot@Alpha\space def
		    /Beta \psk@ThreeDplot@Beta\space def
		    /tMin #1 def
		    /t tMin def
		    /t1 #2 def
		    /dt t1 t sub \psk@ThreeDplot@xPlotpoints\space div def
		    /du #4\space #3\space sub \psk@ThreeDplot@yPlotpoints\space div def
		    /u #3\space \n@Y\space du mul add def
		    /xyz {
			#5
			3 -1 roll               % y z x
			\psk@ThreeDplot@xThreeDunit\space div
			dup                     % y z x x
			neg Alpha cos mul       % y z x (x)
			4 -1 roll               % z x (x) y
			\psk@ThreeDplot@yThreeDunit\space div
			dup                     % z x (x) y y
			5 1 roll                % y z x (x) y
			Alpha sin mul add \pst@number\psxunit mul       % y z x (x2)
			4 1 roll                % (x2) y z x
			Alpha sin mul           % (x2) y z (x)
			3 -1 roll               % (x2) z (x) y
			Alpha cos mul add neg Beta sin mul % (x2) z (x)
			exch                    % (x2) (x) z
			\psk@ThreeDplot@zThreeDunit\space div
			Beta cos mul add \pst@number\psyunit mul        % (x2) (y2)
		    } def
		}%
		\psParamPlotThreeD@iv%
	    }%
	\fi
    \endgroup
    \ignorespaces%
}
\def\psParamPlotThreeD@iii{%
    \addto@pscode{%
	xyz \@nameuse{beginqp@\psplotstyle}
	\psk@ThreeDplot@yPlotpoints\space 1 add {
	    /t tMin def
	    xyz moveto
	    \psk@ThreeDplot@xPlotpoints\space 1 add {
		xyz \@nameuse{doqp@\psplotstyle}
		/t t dt add def
	    } repeat
	    /u u du add def
	} repeat
	/t u1 def
	/u u1 def
	xyz \@nameuse{doqp@\psplotstyle}
    }%
    \@nameuse{endqp@\psplotstyle}%
}
\def\psParamPlotThreeD@iv{%
	\addto@pscode{%
%	    /t tMin def
		mark
	    /n 2 def
		\psk@ThreeDplot@xPlotpoints {
			xyz
    		n 2 roll
    		/n n 2 add def
    		/t t dt add def
		} repeat
		/t t1 def
		xyz
		n 2 roll
    }%
	\@nameuse{endplot@\psplotstyle}%
}
%
% Plot 3D data
%
\def\fileplotThreeD{\def\pst@par{}\pst@object{fileplotThreeD}}
\def\fileplotThreeD@i#1{%
    \pst@killglue
    \begingroup
	\use@par
	\@pstfalse
	\@nameuse{testqp@\psplotstyle}%
	\if@pst
	    \dataplotThreeD@ii{\pst@readfile{#1}}%
	\else
	    \listplotThreeD@ii{\pst@altreadfile{#1}}%
	\fi
    \endgroup
    \ignorespaces%
}
%
% dataplot
%
\def\dataplotThreeD{\def\pst@par{}\pst@object{dataplotThreeD}}
\def\dataplotThreeD@i#1{%
  \pst@killglue
  \begingroup
    \use@par
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \dataplotThreeD@ii{\addto@pscode{#1}}%
    \else
      \listplot@ii{\addto@pscode{#1}}%
    \fi
  \endgroup
  \ignorespaces%
}
\def\dataplotThreeD@ii#1{%
  \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      /Alpha \psk@ThreeDplot@Alpha\space def
      /Beta \psk@ThreeDplot@Beta\space def
      /Dx { /D { Dy } def } def
      /Dy { /D { Dz } def } def
      /Dz { 			% now we have x y z
	3 -1 roll		% y z x
        \psk@ThreeDplot@xThreeDunit\space div
	dup			% y z x x
	neg Alpha cos mul	% y z x (x)
	4 -1 roll		% z x (x) y
	\psk@ThreeDplot@yThreeDunit\space div
	dup			% z x (x) y y
	5 1 roll		% y z x (x) y
	Alpha sin mul add \pst@number\psxunit mul % y z x (x2)
	4 1 roll		% (x2) y z x
	Alpha sin mul		% (x2) y z (x)
	3 -1 roll		% (x2) z (x) y
	Alpha cos mul add neg Beta sin mul % (x2) z (x)
	exch			% (x2) (x) z
	\psk@ThreeDplot@zThreeDunit\space div
	Beta cos mul add \pst@number\psyunit mul % (x2) (y2)
	Do /D { Dx } def } def
      /D { /D { Dx } def } def
      /Do {
        \@nameuse{beginqp@\psplotstyle}%
        /Do { \@nameuse{doqp@\psplotstyle}} def
      } def}%
    #1%
    \addto@pscode{D}%
  \@nameuse{endqp@\psplotstyle}%
}
%
%
\pst@def{ScalePointsThreeD}<%
	counttomark dup dup cvi eq not { exch pop } if
	/m exch def /n m 3 div cvi def
	n { 				% now we have x y z
		3 -1 roll		% y z x
		\psk@ThreeDplot@xThreeDunit\space div
		dup			% y z x x
		neg Alpha cos mul	% y z x (x)
		4 -1 roll		% z x (x) y
		\psk@ThreeDplot@yThreeDunit\space div
		dup			% z x (x) y y
		5 1 roll		% y z x (x) y
		Alpha sin mul add \pst@number\psxunit mul	% y z x (x2)
		4 1 roll		% (x2) y z x
		Alpha sin mul		% (x2) y z (x)
		3 -1 roll		% (x2) z (x) y
		Alpha cos mul add neg Beta sin mul % (x2) z (x)
		exch			% (x2) (x) z
		\psk@ThreeDplot@zThreeDunit\space div
		Beta cos mul add \pst@number\psyunit mul 	% (x2) (y2)
		m 1 sub 1 roll m 1 sub 1 roll /m m 3 sub def } repeat>
%
% listplotThreeD
%
\def\listplotThreeD{\def\pst@par{}\pst@object{listplotThreeD}}
\def\listplotThreeD@i#1{\listplotThreeD@ii{\addto@pscode{#1}}}
\def\listplotThreeD@ii#1{%
	\@nameuse{beginplot@\psplotstyle}%
	\addto@pscode{%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/D {} def mark %
	}%
	#1%
	\addto@pscode{\tx@ScalePointsThreeD}%
	\@nameuse{endplot@\psplotstyle}%
}
%
% adopted from pst-3d
%
\pst@def{TMSave}<%  
  tx@Dict /TMatrix known not { /TMatrix { } def /RAngle { 0 } def } if
  /TMatrix [ TMatrix CM ] cvx def>
%
\pst@def{TMRestore}<%
  CP /TMatrix [ TMatrix setmatrix ] cvx def moveto>
%
\pst@def{TMChange}<%
  \tx@TMSave
  /cp [ currentpoint ] cvx def
  CM
  CP T \tx@STV
  CM matrix invertmatrix 
  matrix concatmatrix 
  exch exec
  concat cp moveto>
%
\def\pstPlanePut{\@ifnextchar[{\pst@PlanePut}{\pst@PlanePut[]}}
\def\pst@PlanePut[#1](#2)#3{{%
	\pst@killglue%
	\setkeys{psset}{origin=lB}%
	\setkeys{psset}{#1}%
	\pstThreeDPut[#1](#2){\ps@Plane{#3}}%
}}
%
\def\ps@Plane{\pst@makebox{\psPlane@}}
\def\psPlane@{%
    \begingroup
	\leavevmode%
    	\hbox{%
%	    \kern\wd\pst@hbox%
	    \pst@Verb{%
		{ [ 1 0
		    /Alpha \psk@ThreeDplot@Alpha\space def
		    /Beta \psk@ThreeDplot@Beta\space def
		    /Delta Beta sin Alpha sin mul Alpha cos atan neg 90 add def 
		    /Gamma Beta sin Alpha cos mul neg Alpha sin atan def 
		    \ifx\psk@ThreeDplot@plane\ThreeDplot@planeXY
			270 Delta sub rotate
			/Rho 90 Gamma add Delta add def
		    \else%
			\ifx\psk@ThreeDplot@plane\ThreeDplot@planeXZ
		    	    270 Delta sub rotate
 			    /Rho 180 Delta add def
			\else%
		    	    Gamma rotate
			    /Rho 90 Gamma sub def
			\fi%
		    \fi%
		    Rho cos Rho sin 0 0 ] concat} \tx@TMChange%
	    }%
	    \box\pst@hbox%
	    \pst@Verb{\tx@TMRestore}%
%	    \kern\ht\pst@hbox%
	}%
    \endgroup%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Utility stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% posStart=Starting point
% length=  Arrow length.
\def\Arrows{\@ifnextchar[{\pst@Arrows}{\pst@Arrows[]}}
\def\pst@Arrows[#1](#2)(#3){{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
		/StartArrow \psk@ThreeDplot@posStart\space def
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/XD StartArrow angleDirectionAB cos mul XA add def
		/YD StartArrow angleDirectionAB sin mul YA add def
		/XF XD LengthArrow angleDirectionAB cos mul add def
		/YF YD LengthArrow angleDirectionAB sin mul add def
		XD YD ){ArrowStart}
	\pnode(! XF YF){ArrowEnd}
	\psset{arrows=->}
	\psline[#1](ArrowStart)(ArrowEnd)%
}}
%
% draw a line (===) outside: #2-----#3=======#4
%
\def\psOutLine{\@ifnextchar[{\pst@ToDrawOut}{\pst@ToDrawOut[]}}
\def\pst@ToDrawOut[#1](#2)(#3)#4{{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/Xend XB LengthArrow angleDirectionAB cos mul add def
		/Yend YB LengthArrow angleDirectionAB sin mul add def
		Xend Yend){#4}
	\psline[#1](#3)(#4)
}}
%
% draw a line (===) before: #4========#2-----#3
%
\def\psBeforeLine{\@ifnextchar[{\pst@BeforeLine}{\pst@BeforeLine[]}}
\def\pst@BeforeLine[#1](#2)(#3)#4{{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/Xstart XA LengthArrow angleDirectionAB cos mul sub def
		/Ystart YA LengthArrow angleDirectionAB sin mul sub def
		Xstart Ystart){#4}
	\psline[#1](#4)(#2)%
}}
%
% intersection de deux droites
% 2 juillet 2001/ rewritten 2003-01-27 Herbert
%
\def\ABinterCD(#1)(#2)(#3)(#4)#5{%
    \pst@getcoor{#1}\pst@tempa
    \pst@getcoor{#2}\pst@tempb
    \pst@getcoor{#3}\pst@tempc
    \pst@getcoor{#4}\pst@tempd
\pnode(!%
    /YA \pst@tempa exch pop \pst@number\psyunit div def
    /XA \pst@tempa pop \pst@number\psxunit div def
    /YB \pst@tempb exch pop \pst@number\psyunit div def
    /XB \pst@tempb pop \pst@number\psxunit div def
    /YC \pst@tempc exch pop \pst@number\psyunit div def
    /XC \pst@tempc pop \pst@number\psxunit div def
    /YD \pst@tempd exch pop \pst@number\psyunit div def
    /XD \pst@tempd pop \pst@number\psxunit div def
    /dY1 YB YA sub def
    /dX1 XB XA sub def
    /dY2 YD YC sub def
    /dX2 XD XC sub def
    dX1 abs 0.01 lt {
	/m2 dY2 dX2 div def
	XA dup XC sub m2 mul YC add 
    }{
	dX2 abs 0.01 lt {
	    /m1 dY1 dX1 div def
	    XC dup XA sub m1 mul YA add 
	}{%
	    /m1 dY1 dX1 div def
	    /m2 dY2 dX2 div def
	    m1 XA mul m2 XC mul sub YA sub YC add m1 m2 sub div dup
	    XA sub m1 mul YA add 
	} ifelse
    } ifelse ){#5}
}
%
% draw a parallel line
%     #2---------#3
%         #4----------#5(new)  
\def\Parallel{\@ifnextchar[{\pst@Parallel}{\pst@Parallel[]}}
\def\pst@Parallel[#1](#2)(#3)(#4)#5{{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pst@getcoor{#4}\pst@tempc
	\pnode(!%
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		\pst@tempc /YC exch \pst@number\psyunit div def
		/XC exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/XstartParallel XC LengthArrow angleDirectionAB cos mul add def
		/YstartParallel YC LengthArrow angleDirectionAB sin mul add def
		XstartParallel YstartParallel){#5}
	\psline[#1](#4)(#5)
}}
%
% arrowLine[options](A)(B){n}
% #2---->---->---->---->----#3  #4-arrows inside
\def\arrowLine{\@ifnextchar[{\pst@arrowLine}{\pst@arrowLine[]}}
\def\pst@arrowLine[#1](#2)(#3)#4{{%
	\setkeys{psset}{arrowsize=4pt,arrows=->}% the defaults
	\setkeys{psset}{#1}%
	\def\pst@ThreeDplot@n{#4}
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
	    	/YA \pst@tempa exch pop \pst@number\psyunit div def
		/XA \pst@tempa pop \pst@number\psxunit div def
		/YB \pst@tempb exch pop \pst@number\psyunit div def
		/XB \pst@tempb pop \pst@number\psxunit div def
		/dY YB YA sub \pst@ThreeDplot@n\space 1 add div def
		/dX XB XA sub \pst@ThreeDplot@n\space 1 add div def
		/Alpha dY dX atan def
		/dYOffset \psk@ThreeDplot@arrowOffset\space Alpha sin mul def
		/dXOffset \psk@ThreeDplot@arrowOffset\space Alpha cos mul def
		XA YA ){tempArrowC}
	\multido{\i=1+1}{#4}{%
		\pnode(!%
			XA dX \i\space mul add dXOffset add
			YA dY \i\space mul add dYOffset add){tempArrowB}
		\psline(tempArrowC)(tempArrowB)
		\pnode(tempArrowB){tempArrowC}
    	}
	\psline[arrows=-](tempArrowB)(#3)
}}
%
%   #1------#3------#2
\def\nodeBetween(#1)(#2)#3{%    Herbert 2003/01/05
    \pst@getcoor{#1}\pst@tempa
    \pst@getcoor{#2}\pst@tempb
    \pnode(!%
	/XA \pst@tempa pop \pst@number\psxunit div def
	/YA \pst@tempa exch pop \pst@number\psyunit div def
	/XB \pst@tempb pop \pst@number\psxunit div def
	/YB \pst@tempb exch pop \pst@number\psyunit div def
	XB XA add 2 div YB YA add 2 div){#3}
}
%
% rotateNode(A)
% (A) the node
% #2  the angle
% Herbert Voss <voss@perce.de> 2003-01-26
\def\rotateNode{\pst@rotateNode}
\def\pst@rotateNode(#1)#2{{%
    \pst@getcoor{#1}\pst@tempa
    \def\pst@ThreeDplot@angle{#2}	% the rotating angle
    \pnode(!%
    	/YA \pst@tempa exch pop \pst@number\psyunit div def
	/XA \pst@tempa pop \pst@number\psxunit div def
	YA 0 eq XA 0 eq and {0 0}{
	    /r XA dup mul YA dup mul add sqrt def
	    /AlphaOld YA XA atan def
	    /AlphaNew AlphaOld \pst@ThreeDplot@angle\space add def
	    r AlphaNew cos mul r AlphaNew sin mul
	} ifelse ){temp}
    \pnode(temp){#1}
}}
%
\def\rotateTriangle{\pst@rotateTriangle}
\def\pst@rotateTriangle(#1)(#2)(#3)#4{{%
    \rotateNode(#1){#4}
    \rotateNode(#2){#4}
    \rotateNode(#3){#4}
}}
%
\def\rotateFrame{\pst@rotateFrame}
\def\pst@rotateFrame(#1)(#2)(#3)(#4)#5{{%
    \rotateNode(#1){#5}
    \rotateNode(#2){#5}
    \rotateNode(#3){#5}
    \rotateNode(#4){#5}
}}
\catcode`\@=\PstAtCode\relax
%
%% END: pst-3dplot.tex
\endinput

%% CHANGE LOG %%
%
% 1.2b	bugfix for adding vectors with decinmal length
% 1.2a	disable the loading of pstcol.sty


==> pst-vue3d.tex <==
%%
%% This is file `pst-vue3d.tex',
%% 
%% IMPORTANT NOTICE:
%% 
%% Package `pst-vue3d.tex'
%%
%% Manuel Luque <Mluque5130@aol.com> (France)
%%
%% 2003/10/17
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-vue3d' is a PSTricks package to define 3d views
%%
\def\fileversion{0.4}%
\def\filedate{2003/10/17}%
\message{`PST-VUE3D v\fileversion, \filedate\space (Manuel LUQUE)}%
\csname PSTVueTroisDLoaded\endcsname
\let\PSTVueTroisDLoaded\endinput
% Require PSTricks and pst-node packages
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
% DPC interface to the `keyval' package (until keyval based version of PSTricks)
\input pst-key.tex
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor

\pstheader{3D.pro}
%%%%
\SpecialCoor
\makeatletter
\define@key{psset}{scale}{\edef\psk@TroisD@scale{#1}} % echelle
\define@key{psset}{RotX}{\edef\psk@TroisD@RotX{#1}} % rotation autour de Ox en degrés
\define@key{psset}{RotY}{\edef\psk@TroisD@RotY{#1}} % rotation autour de Oy en degrés
\define@key{psset}{RotZ}{\edef\psk@TroisD@RotZ{#1}} % rotation autour de OZ en degrés
\define@key{psset}{A}{\edef\psk@TroisD@A{#1}} % double  d'une arête du parallèlépipède
\define@key{psset}{B}{\edef\psk@TroisD@B{#1}} % double  d'une arête du parallèlépipède
\define@key{psset}{C}{\edef\psk@TroisD@C{#1}} % double  de l'arête du parallèlépipède
\define@key{psset}{CX}{\edef\psk@TroisD@Xc{#1}} % abscisse du centre du paarallèlépipède
\define@key{psset}{CY}{\edef\psk@TroisD@Yc{#1}} % ordonnée centre du cube
\define@key{psset}{CZ}{\edef\psk@TroisD@Zc{#1}} % cote centre du cube
\define@key{psset}{Rtetraedre}{\edef\psk@TroisD@Rtetraedre{#1}} % Rayon du cercle tétraèdre
\define@key{psset}{ColorFaceA}{\edef\psk@TroisD@TetraedreColorFaceA{#1}} % couleur de la face A du tétraèdre
\define@key{psset}{ColorFaceB}{\edef\psk@TroisD@TetraedreColorFaceB{#1}} % couleur de la face B du tétraèdre
\define@key{psset}{ColorFaceC}{\edef\psk@TroisD@TetraedreColorFaceC{#1}} % couleur de la face C du tétraèdre
\define@key{psset}{ColorFaceD}{\edef\psk@TroisD@TetraedreColorFaceD{#1}} % couleur de la face D du tétraèdre
\define@key{psset}{ColorFaceE}{\edef\psk@TroisD@TetraedreColorFaceE{#1}} % couleur de la face D du tétraèdre
\define@key{psset}{fracHcone}{\edef\psk@TroisD@fracHcone{#1}} % fraction de la hauteur du cone
\define@key{psset}{Hpyramide}{\edef\psk@TroisD@Hpyramide{#1}} % hauteur pyramide
%
\define@key{psset}{normaleLongitude}{\edef\psk@TroisD@normaleLongitude{#1}} % coordonnées angulaires de la normale
\define@key{psset}{normaleLatitude}{\edef\psk@TroisD@normaleLatitude{#1}} % coordonnées angulaires de la normale
\define@key{psset}{Xorigine}{\edef\psk@TroisD@Xorigine{#1}} % coordonnées de la nouvelle origine
\define@key{psset}{Yorigine}{\edef\psk@TroisD@Yorigine{#1}} % coordonnées de la nouvelle origine
\define@key{psset}{Zorigine}{\edef\psk@TroisD@Zorigine{#1}} % coordonnées de la nouvelle origine
\define@key{psset}{Xmax}{\edef\psk@TroisD@Xmax{#1}} % en cm
\define@key{psset}{Xmin}{\edef\psk@TroisD@Xmin{#1}} % en cm
\define@key{psset}{Ymax}{\edef\psk@TroisD@Ymax{#1}} % en cm
\define@key{psset}{Ymin}{\edef\psk@TroisD@Ymin{#1}} % en cm
\define@key{psset}{pas}{\edef\psk@TroisD@pas{#1}} % en cm résolution du tracé
\define@key{psset}{grille}{\edef\psk@TroisD@grille{#1}} % Pas de la grille en cm
%
\define@key{psset}{THETA}{\edef\psk@TroisD@Theta{#1}}
\define@key{psset}{PHI}{\edef\psk@TroisD@Phi{#1}}
\define@key{psset}{DeltaTHETA}{\edef\psk@TroisD@DeltaTheta{#1}}
\define@key{psset}{DeltaPHI}{\edef\psk@TroisD@DeltaPhi{#1}}
\define@key{psset}{PortionSphereTHETA}{\edef\psk@TroisD@PortionSphereTHETA{#1}}
\define@key{psset}{PortionSpherePHI}{\edef\psk@TroisD@PortionSpherePHI{#1}}
\define@key{psset}{PhiCercle}{\edef\psk@TroisD@PhiCercle{#1}}
\define@key{psset}{ThetaMeridien}{\edef\psk@TroisD@ThetaMeridien{#1}}
\define@key{psset}{Dobs}{\edef\psk@TroisD@Dobs{#1}}
\define@key{psset}{Decran}{\edef\psk@TroisD@Ecran{#1}}
\setkeys{psset}{THETA=30,PHI=10,Dobs=100,Decran=10}
%
\setkeys{psset}{normaleLongitude=45,%
                normaleLatitude=45,%
                PhiCercle=0,%
                ThetaMeridien=0,%
                Xorigine=0,%
                Yorigine=0,%
                Zorigine=0,%
                Xmax=50,%
                Ymax=50,%
                Xmin=-50,%
                Ymin=-50,%
                pas=1,%
                grille=10,%
                normaleLongitude=45,%
                normaleLatitude=45,%
                scale=1,%
                RotX=0,RotY=0,RotZ=0,%
                A=10,B=10,C=10,%
                CX=0,CY=0,CZ=0,%
                Rtetraedre=5,%
                ColorFaceD=cyan,ColorFaceA=magenta,ColorFaceB=red,ColorFaceC=blue,ColorFaceE=yellow,%
                fracHcone=1,Hpyramide=5,%
                DeltaTHETA=10,DeltaPHI=10,%
                PortionSphereTHETA=0,PortionSpherePHI=0}
% ajout du 28 août 2003
% colorier au choix les faces du cube
\define@key{psset}{CubeColorFaceOne}{\edef\psk@TroisD@CubeColorFaceOne{#1}} % couleur de la face 1 du cube
\define@key{psset}{CubeColorFaceTwo}{\edef\psk@TroisD@CubeColorFaceTwo{#1}} % couleur de la face 2 du cube
\define@key{psset}{CubeColorFaceThree}{\edef\psk@TroisD@CubeColorFaceThree{#1}} % couleur de la face 3 du cube
\define@key{psset}{CubeColorFaceFour}{\edef\psk@TroisD@CubeColorFaceFour{#1}} % couleur de la face 4 du cube
\define@key{psset}{CubeColorFaceFive}{\edef\psk@TroisD@CubeColorFaceFive{#1}} % couleur de la face 5 du cube
\define@key{psset}{CubeColorFaceSix}{\edef\psk@TroisD@CubeColorFaceSix{#1}} % couleur de la face 6 du cube
\psset{CubeColorFaceOne=1 1 0,%
       CubeColorFaceTwo=0.9 0.9 0,%
       CubeColorFaceThree=0.8 0.8 0,%
       CubeColorFaceFour=0.7 0.7 0,%
       CubeColorFaceFive=0.65 0.65 0,%
       CubeColorFaceSix=0.75 0.75 0}
% fin 28 août 2003
%
\def\variablesTroisD{%
 0 0 translate
    /reduction \psk@TroisD@scale\space def
    /RotX \psk@TroisD@RotX\space def
    /RotY \psk@TroisD@RotY\space def
    /RotZ \psk@TroisD@RotZ\space def
    /CX \psk@TroisD@Xc\space def
    /CY \psk@TroisD@Yc\space def
    /CZ \psk@TroisD@Zc\space def
    /A \psk@TroisD@A\space def
    /B \psk@TroisD@B\space def
    /C \psk@TroisD@C\space def
    /RayonBaseTetraedre \psk@TroisD@Rtetraedre\space def
    /Hpyramide \psk@TroisD@Hpyramide\space def
    /Rpoint A 4 div def
    /nTheta \psk@TroisD@normaleLongitude\space def
    /nPhi \psk@TroisD@normaleLatitude\space def
    /S1 \psk@TroisD@normaleLongitude\space sin def
    /C1 \psk@TroisD@normaleLongitude\space cos def
    /S2 \psk@TroisD@normaleLatitude\space sin def
    /C2 \psk@TroisD@normaleLatitude\space cos def
    /THETA \psk@TroisD@Theta\space def
    /PHI \psk@TroisD@Phi\space def
    /dTHETA \psk@TroisD@DeltaTheta\space def
    /dPHI \psk@TroisD@DeltaPhi\space def
    /psTHETA \psk@TroisD@PortionSphereTHETA\space def
    /psPHI \psk@TroisD@PortionSpherePHI\space def
    /PhiCercle \psk@TroisD@PhiCercle\space def
    /ThetaMeridien \psk@TroisD@ThetaMeridien\space def
    /Dobs \psk@TroisD@Dobs\space def
    /DScreen \psk@TroisD@Ecran\space def
    /Sin1 THETA sin def
    /Sin2 PHI sin def
    /Cos1 THETA cos def
    /Cos2 PHI cos def
    /Cos1Sin2 Cos1 Sin2 mul def
    /Sin1Sin2 Sin1 Sin2 mul def
    /Cos1Cos2 Cos1 Cos2 mul def
    /Sin1Cos2 Sin1 Cos2 mul def
    /XpointVue Dobs Cos1Cos2 mul def
    /YpointVue Dobs Sin1Cos2 mul def
    /ZpointVue Dobs Sin2 mul def
    /M11 RotZ cos RotY cos mul def
    /M12 RotZ cos RotY sin mul RotX sin mul
         RotZ sin RotX cos mul sub def
    /M13 RotZ cos RotY sin mul RotX cos mul
         RotZ sin RotX sin mul add def
    /M21 RotZ sin RotY cos mul def
    /M22 RotZ sin RotY sin RotX sin mul mul
         RotZ cos RotX cos mul add def
    /M23 RotZ sin RotY sin mul RotX cos mul
         RotZ cos RotX sin mul sub def
    /M31 RotY sin neg def
    /M32 RotX sin RotY cos mul def
    /M33 RotX cos RotY cos mul def
 }%

\def\Cube{\pst@object{Cube}}
\def\Cube@i{\@ifnextchar[{\Cube@do}{\Cube@do[]}}
\def\Cube@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
/CubeColorFaceOne {\psk@TroisD@CubeColorFaceOne} def
/CubeColorFaceTwo {\psk@TroisD@CubeColorFaceTwo} def
/CubeColorFaceThree {\psk@TroisD@CubeColorFaceThree} def
/CubeColorFaceFive {\psk@TroisD@CubeColorFaceFive} def
/CubeColorFaceFour {\psk@TroisD@CubeColorFaceFour} def
/CubeColorFaceSix {\psk@TroisD@CubeColorFaceSix} def
tx@3DDict begin
Cube
end
}% fin du code ps
\end@ClosedObj
}}
%
\def\Die{\pst@object{Die}}
\def\Die@i{\@ifnextchar[{\Die@do}{\Die@do[]}}
\def\Die@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
/CubeColorFaceOne {\psk@TroisD@CubeColorFaceOne} def
/CubeColorFaceTwo {\psk@TroisD@CubeColorFaceTwo} def
/CubeColorFaceThree {\psk@TroisD@CubeColorFaceThree} def
/CubeColorFaceFive {\psk@TroisD@CubeColorFaceFive} def
/CubeColorFaceFour {\psk@TroisD@CubeColorFaceFour} def
/CubeColorFaceSix {\psk@TroisD@CubeColorFaceSix} def
tx@3DDict begin
Cube
PointsDie
end
}% fin du code ps
\end@ClosedObj}}
%
\def\SphereThreeD{\pst@object{SphereThreeD}}
\def\SphereThreeD@i{\@ifnextchar[{\SphereThreeD@do}{\SphereThreeD@do[]}}
\def\SphereThreeD@do[#1]#2{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
    /increment 10 def
tx@3DDict begin
/condition {PSfacette 0 le} def
/departPhi -90 def
MaillageSphere
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj}}
% % fin de la commande PSTricks
%
% 2décembre 2002
%
\def\SphereInverse{\pst@object{SphereInverse}}
\def\SphereInverse@i{\@ifnextchar[{\SphereInverse@do}{\SphereInverse@do[]}}
\def\SphereInverse@do[#1]#2{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
    /increment 10 def
tx@3DDict begin
/condition {PSfacette 0 ge} def
/departPhi -90 def
MaillageSphere
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj}}
% % fin de la commande PSTricks
% fin 2 décembre 2002
%
\def\SphereCercle{\pst@object{SphereCercle}}
\def\SphereCercle@i{\@ifnextchar[{\SphereCercle@do}{\SphereCercle@do[]}}
\def\SphereCercle@do[#1]#2{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
tx@3DDict begin
0 2 360 {
    /ThetaEquateur exch def
    /Xpoint Rsphere ThetaEquateur cos mul PhiCercle cos mul def
    /Ypoint Rsphere ThetaEquateur sin mul PhiCercle cos mul def
    /Zpoint Rsphere PhiCercle sin mul def
CalculsPointsAfterTransformations
% rayon de las sphère (normale)
    /nXfacette Xabscisse CX sub def
    /nYfacette Yordonnee CY sub def
    /nZfacette Zcote CZ sub def
% rayon vers point de vue
    /RXvue Xabscisse XpointVue sub def
    /RYvue Yordonnee YpointVue sub def
    /RZvue Zcote ZpointVue sub def
% test de visibilité
    /PSPoint RXvue nXfacette mul
    RYvue nYfacette mul add
    RZvue nZfacette mul add
    def
PSPoint 0 le{
newpath
    CalcCoordinates
0.5 0 360 arc
closepath
fill
} if
%lineto
} for
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
}}
%
%
\def\SphereMeridien{\pst@object{SphereMeridien}}
\def\SphereMeridien@i{\@ifnextchar[{\SphereMeridien@do}{\SphereMeridien@do[]}}
\def\SphereMeridien@do[#1]#2{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
tx@3DDict begin
0 2 360 {
    /PhiCercle exch def
    /Xpoint Rsphere ThetaMeridien cos mul PhiCercle cos mul def
    /Ypoint Rsphere ThetaMeridien sin mul PhiCercle cos mul def
    /Zpoint Rsphere PhiCercle sin mul def
CalculsPointsAfterTransformations
% rayon de las sphère (normale)
    /nXfacette Xabscisse CX sub def
    /nYfacette Yordonnee CY sub def
    /nZfacette Zcote CZ sub def
% rayon vers point de vue
    /RXvue Xabscisse XpointVue sub def
    /RYvue Yordonnee YpointVue sub def
    /RZvue Zcote ZpointVue sub def
% test de visibilité
    /PSPoint RXvue nXfacette mul
    RYvue nYfacette mul add
    RZvue nZfacette mul add
    def
PSPoint 0 le{
newpath
    CalcCoordinates
0.5 0 360 arc
closepath
fill
} if
%lineto
} for
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
}}
%
\def\CylindreThreeD{\pst@object{CylindreThreeD}}
\def\CylindreThreeD@i{\@ifnextchar[{\CylindreThreeD@do}{\CylindreThreeD@do[]}}
\def\CylindreThreeD@do[#1]#2#3{{%
% Le centre de la base sera placé avec
% les paramètres CX,CY et CZ
% #2 rayon
% #3 hauteur
% on peut ensuite faire tourner le cylindre
% avec RotX, RotY et RotZ
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rcylindre #2 def
    /Hcylindre #3 def
    /incrementANGLE 10 def
    /incrementHAUTEUR Hcylindre 5 div def
tx@3DDict begin
CylinderThreeD
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}% % fin de la commande PSTricks
%
%
\def\LineThreeD{\pst@object{LineThreeD}}
\def\LineThreeD@i{\@ifnextchar[{\LineThreeD@do}{\LineThreeD@do[]}}
\def\LineThreeD@do[#1](#2,#3,#4)(#5,#6,#7){{%
% (#2,#3,#4) coordonnées du point1
% (#5,#6,#7) coordonnées du point2
\pst@killglue
\setkeys{psset}{#1}%
\begin@OpenObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
/X1 #2 def
/Y1 #3 def
/Z1 #4 def
/X2 #5 def
/Y2 #6 def
/Z2 #7 def
tx@3DDict begin
/TableauxPoints [
0 0.01 1.01 { % k
    /K exch def
    [
    /Zcote K Z2 mul 1 K sub Z1 mul add def
    /Xabscisse K X2 mul 1 K sub X1 mul add def
    /Yordonnee K Y2 mul 1 K sub Y1 mul add def
    CalcCoordinates ]
    } for
 ] def
 TableauxPoints 0 get aload pop moveto
 0 1 100 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
% fin du tracé de la ligne
end
 }% fin du code ps
 \end@OpenObj
 }}% % fin de la commande PSTricks
%
%
%
% transformation d'un point
\def\PointThreeD{\@ifnextchar[{\pst@PointThreeD}{\pst@PointThreeD[]}}
%
\def\pst@PointThreeD[#1](#2,#3,#4)#5{{%
%(#2,#3,#4) coordonnées
% #5 nom attribué au point
\setkeys{psset}{#1}
\pnode(!
\variablesTroisD
 /Zcote #4 def
 /Xabscisse #2 def
 /Yordonnee #3 def
tx@3DDict begin
  formulesTroisD
 Xi reduction mul Yi reduction mul
 end){#5}}}
%
% transformation d'un point
\def\PointLongitudeLatitude{\@ifnextchar[{\pst@PointLongitudeLatitude}{\pst@PointLongitudeLatitude[]}}
%
\def\pst@PointLongitudeLatitude[#1]#2#3#4#5{{%
% #2 radius
% #3 longitude
% #4 latitude
% #5 nom attribué au point
\pst@killglue
\setkeys{psset}{#1}%
\pnode(!
\variablesTroisD
/Radius #2 def
/longitude #3 def
/latitude #4 def
 /Zcote Radius latitude sin mul def
 /Xabscisse Radius longitude cos mul latitude cos mul def
 /Yordonnee Radius longitude sin mul latitude cos mul def
tx@3DDict begin
formulesTroisD
 Xi reduction mul Yi reduction mul
 end){#5}
}}
%
\def\Tetraedre{\pst@object{Tetraedre}}
\def\Tetraedre@i{\@ifnextchar[{\Tetraedre@do}{\Tetraedre@do[]}}
\def\Tetraedre@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
tx@3DDict begin
Tetraedre
end
}% fin du code ps
\end@ClosedObj
}}
%
%
% pyramide
%
\def\FaceSAB{\pst@object{FaceSAB}}
\def\FaceSAB@i{\@ifnextchar[{\FaceSABC@do}{\FaceSAB@do[]}}
\def\FaceSAB@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
tx@3DDict begin
SommetsPyramide
 PSAB 0 le { %
reduction reduction scale
newpath
1 setlinejoin
    /Xabscisse XS def
    /Yordonnee YS def
    /Zcote ZS def
    CalcCoordinates
     moveto
    /Xabscisse XA def
    /Yordonnee YA def
    /Zcote ZA def
    CalcCoordinates
    lineto
    /Xabscisse XB def
    /Yordonnee YB def
    /Zcote ZB def
    CalcCoordinates
    lineto
closepath
} if
end
}% fin du code ps
\end@ClosedObj
}}
%
\def\FaceSBC{\pst@object{FaceSBC}}
\def\FaceSBC@i{\@ifnextchar[{\FaceSBC@do}{\FaceSBC@do[]}}
\def\FaceSBC@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
tx@3DDict begin
SommetsPyramide
 PSBC 0 le { %
reduction reduction scale
newpath
1 setlinejoin
    /Xabscisse XS def
    /Yordonnee YS def
    /Zcote ZS def
    CalcCoordinates
     moveto
    /Xabscisse XB def
    /Yordonnee YB def
    /Zcote ZB def
    CalcCoordinates
    lineto
     /Xabscisse XC def
    /Yordonnee YC def
    /Zcote ZC def
    CalcCoordinates
    lineto
closepath
} if
end
}% fin du code ps
\end@ClosedObj
}}
%
%
\def\FaceSCD{\pst@object{FaceSCD}}
\def\FaceSCD@i{\@ifnextchar[{\FaceSCD@do}{\FaceSCD@do[]}}
\def\FaceSCD@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
tx@3DDict begin
SommetsPyramide
PSCD 0 le { %
reduction reduction scale
newpath
1 setlinejoin
    /Xabscisse XS def
    /Yordonnee YS def
    /Zcote ZS def
    CalcCoordinates
     moveto
    /Xabscisse XC def
    /Yordonnee YC def
    /Zcote ZC def
    CalcCoordinates
    lineto
    /Xabscisse XD def
    /Yordonnee YD def
    /Zcote ZD def
    CalcCoordinates
    lineto
closepath
} if
end
}% fin du code ps
\end@ClosedObj
}}
%
\def\FaceSDA{\pst@object{FaceSDA}}
\def\FaceSDA@i{\@ifnextchar[{\FaceSDA@do}{\FaceSDA@do[]}}
\def\FaceSDA@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
tx@3DDict begin
SommetsPyramide
 PSDA 0 le { %
reduction reduction scale
newpath
1 setlinejoin
    /Xabscisse XS def
    /Yordonnee YS def
    /Zcote ZS def
    CalcCoordinates
     moveto
    /Xabscisse XD def
    /Yordonnee YD def
    /Zcote ZD def
    CalcCoordinates
    lineto
    /Xabscisse XA def
    /Yordonnee YA def
    /Zcote ZA def
    CalcCoordinates
    lineto
closepath
} if
end
}% fin du code ps
\end@ClosedObj
}}
%
\def\FaceABCD{\pst@object{FaceABCD}}
\def\FaceABCD@i{\@ifnextchar[{\FaceABCD@do}{\FaceABCD@do[]}}
\def\FaceABCD@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
tx@3DDict begin
SommetsPyramide
 PSABCD 0 le { %
reduction reduction scale
newpath
1 setlinejoin
    /Xabscisse XA def
    /Yordonnee YA def
    /Zcote ZA def
    CalcCoordinates
     moveto
    /Xabscisse XB def
    /Yordonnee YB def
    /Zcote ZB def
    CalcCoordinates
    lineto
    /Xabscisse XC def
    /Yordonnee YC def
    /Zcote ZC def
    CalcCoordinates
    lineto
    /Xabscisse XD def
    /Yordonnee YD def
    /Zcote ZD def
    CalcCoordinates
    lineto
closepath
} if
end
}% fin du code ps
\end@ClosedObj
}}
%
\def\Pyramide{\pst@object{Pyramide}}
\def\Pyramide@i{\@ifnextchar[{\Pyramide@do}{\Pyramide@do[]}}
\def\Pyramide@do[#1]{{%
\FaceSAB[fillcolor=\psk@TroisD@TetraedreColorFaceA]%
\FaceSBC[fillcolor=\psk@TroisD@TetraedreColorFaceB]%
\FaceSCD[fillcolor=\psk@TroisD@TetraedreColorFaceC]%
\FaceSDA[fillcolor=\psk@TroisD@TetraedreColorFaceD]%
\FaceABCD[fillcolor=\psk@TroisD@TetraedreColorFaceE]%
}}
%
%
\def\ConeThreeD{\pst@object{ConeThreeD}}
\def\ConeThreeD@i{\@ifnextchar[{\ConeThreeD@do}{\ConeThreeD@do[]}}
\def\ConeThreeD@do[#1]#2#3{{%
% Le centre de la base sera placé avec
% les paramètres CX,CY et CZ
% #2 rayon
% #3 hauteur
% on peut ensuite faire tourner le cylindre
% avec RotX, RotY et RotZ
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
    /fracHcone \psk@TroisD@fracHcone\space def
% fraction de la hauteur du cone 0<fracHcone<1
reduction reduction scale
    /Rcone #2 def
    /Hcone #3 def
    /AngleCone Rcone Hcone atan def
    /TanAngleCone AngleCone dup sin exch cos div def
    /incrementANGLE 10 def
    /incrementHAUTEUR Hcone fracHcone mul  5 div def
tx@3DDict begin
newpath
0 incrementANGLE 360 {%
    /theta exch def
 0 incrementHAUTEUR Hcone fracHcone mul incrementHAUTEUR sub {%
    /H exch def
 % normale à la facette
    /nXfacette Hcone AngleCone dup sin exch cos mul theta incrementANGLE 2 div add cos mul
    mul def
    /nYfacette Hcone AngleCone dup sin exch cos mul theta incrementANGLE 2 div add sin mul
    mul def
    /nZfacette Hcone AngleCone sin dup mul mul def
    /Xpoint nXfacette def
    /Ypoint nYfacette def
    /Zpoint nZfacette def
CalculsPointsAfterTransformations
    /nXfacette Xabscisse CX sub def
    /nYfacette Yordonnee CY sub def
    /nZfacette Zcote CZ sub def
%
    /OK Hcone H sub TanAngleCone mul def
    /Xpoint OK theta cos mul def
    /Ypoint OK theta sin mul def
    /Zpoint H def
CalculsPointsAfterTransformations
    /Xfacette Xabscisse  def
    /Yfacette Yordonnee  def
    /Zfacette Zcote def
    CalcCoordinates
     moveto
% coordonnées du centre de la facette
    /OK Hcone H incrementHAUTEUR 2 div add sub TanAngleCone mul def
    /Xpoint OK theta incrementANGLE 2 div add cos mul def
    /Ypoint OK theta incrementANGLE 2 div add sin mul def
    /Zpoint H incrementHAUTEUR 2 div add def
CalculsPointsAfterTransformations
    /XcentreFacette Xabscisse  def
    /YcentreFacette Yordonnee  def
    /ZcentreFacette Zcote def
% rayon vers point de vue
    /RXvue XcentreFacette XpointVue sub def
    /RYvue YcentreFacette YpointVue sub def
    /RZvue ZcentreFacette ZpointVue sub def
% test de visibilité
    /PSfacette nXfacette RXvue mul
    nYfacette RYvue mul add
    nZfacette RZvue mul add
    def
PSfacette 0 le {
theta 1 theta incrementANGLE add {%
    /theta1 exch def
    /OK Hcone H sub TanAngleCone mul def
    /Xpoint OK theta1 cos mul def
    /Ypoint OK theta1 sin mul def
    /Zpoint H def
CalculsPointsAfterTransformations
    CalcCoordinates
    lineto
    } for
H 1 H incrementHAUTEUR add {
    /H1 exch def
    /OK Hcone H1 sub TanAngleCone mul def
    /Xpoint OK theta incrementANGLE add cos mul def
    /Ypoint OK theta incrementANGLE add sin mul def
    /Zpoint H1 def
CalculsPointsAfterTransformations
    CalcCoordinates
    lineto
    } for
theta incrementANGLE add -1 theta {%
    /theta1 exch def
    /OK Hcone H incrementHAUTEUR add sub TanAngleCone mul def
    /Xpoint OK theta1 cos mul def
    /Ypoint OK theta1 sin mul def
    /Zpoint H incrementHAUTEUR add def
CalculsPointsAfterTransformations
    CalcCoordinates
    lineto
    } for
H incrementHAUTEUR add -1 H {
    /H1 exch def
    /OK Hcone H1 sub TanAngleCone mul def
    /Xpoint OK theta cos mul def
    /Ypoint OK theta sin mul def
    /Zpoint H1 def
CalculsPointsAfterTransformations
    CalcCoordinates
    lineto
    } for
} if
} for
} for
% centre de la base inférieure après transformations
    /CxFaceInf CX def
    /CyFaceInf CY def
    /CzFaceInf CZ def
% modification du 16/11/2002
%    /Xpoint CxFaceInf def
%    /Ypoint CyFaceInf def
%    /Zpoint CzFaceInf def
    /Xpoint 0 def
    /Ypoint 0 def
    /Zpoint 0 def
% fin modification du 16/11/2002
CalculsPointsAfterTransformations
    /CxBaseInf Xabscisse def
    /CyBaseInf Yordonnee def
    /CzBaseInf Zcote def
% centre de la base supérieure avant transformations
    /CxFaceSup 0 def
    /CyFaceSup 0 def
    /CzFaceSup Hcone fracHcone mul def
% Sommet du cone
    /Xpoint 0 def
    /Ypoint 0 def
    /Zpoint Hcone def
CalculsPointsAfterTransformations
    /XsommetCone Xabscisse def
    /YsommetCone Yordonnee def
    /ZsommetCone Zcote def
% Normale extérieure à la base inférieure
    /nXBaseInf CxFaceInf XsommetCone sub def
    /nYBaseInf CyFaceInf YsommetCone sub def
    /nZBaseInf CzFaceInf ZsommetCone sub def
% centre de la base supérieure
    /Xpoint CxFaceSup def
    /Ypoint CyFaceSup def
    /Zpoint CzFaceSup def
CalculsPointsAfterTransformations
    /CxBaseSup Xabscisse def
    /CyBaseSup Yordonnee def
    /CzBaseSup Zcote def
% Normale extérieure à la base supérieure
    /nXBaseSup XsommetCone CxFaceSup sub def
    /nYBaseSup YsommetCone CyFaceSup sub def
    /nZBaseSup ZsommetCone CzFaceSup sub def
% rayon vers point de vue
    /RXvueSup CxBaseSup XpointVue sub def
    /RYvueSup CyBaseSup YpointVue sub def
    /RZvueSup CzBaseSup ZpointVue sub def
    /RXvueInf CxBaseInf XpointVue sub def
    /RYvueInf CyBaseInf YpointVue sub def
    /RZvueInf CzBaseInf ZpointVue sub def
% Visibilité de la base inférieure
    /PSbaseInfCone nXBaseInf RXvueInf mul
                nYBaseInf RYvueInf mul add
                nZBaseInf RZvueInf mul add def
% Visibilité de la base supérieure
    /PSbaseSupCone nXBaseSup RXvueSup mul
                nYBaseSup RYvueSup mul add
                nZBaseSup RZvueSup mul add def
PSbaseInfCone 0 le {
/TableauxPoints [
0 1 359 {% on décrit le cercle
    /theta exch def [
    /Xpoint Rcone theta cos mul def
    /Ypoint Rcone theta sin mul def
    /Zpoint 0 def
CalculsPointsAfterTransformations
    CalcCoordinates ]
    } for
    ] def
gsave
newpath
 TableauxPoints 0 get aload pop moveto
0 1 359 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
0.7 setgray
closepath
fill
grestore
 } if
PSbaseSupCone 0 le {
/TableauxPoints [
0 1 359 {% on décrit le cercle
    /theta exch def [
    /OK Hcone 1 fracHcone sub mul TanAngleCone mul def
    /Xpoint OK theta cos mul def
    /Ypoint OK theta sin mul def
    /Zpoint Hcone fracHcone mul def
CalculsPointsAfterTransformations
    CalcCoordinates ]
    } for
    ] def
gsave
newpath
 TableauxPoints 0 get aload pop moveto
0 1 359 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
0.7 setgray
closepath
fill
grestore
 } if
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}%
%
\def\CircleThreeD{\pst@object{CircleThreeD}}
\def\CircleThreeD@i{\@ifnextchar[{\CircleThreeD@do}{\CircleThreeD@do[]}}
\def\CircleThreeD@do[#1]#2{{%
% #2 rayon du cercle
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
/Rcercle #2 def
\variablesTroisD
/XO' \psk@TroisD@Xorigine\space def
/YO' \psk@TroisD@Yorigine\space def
/ZO' \psk@TroisD@Zorigine\space def
tx@3DDict begin
reduction reduction scale
/TableauxPoints [
0 1 359 {% on décrit le cercle
    /Angle exch def [
    /Xcercle Rcercle Angle cos mul def
    /Ycercle Rcercle Angle sin mul def
    /Xabscisse Xcercle S1 mul Ycercle S2 C1 mul mul add XO' add
    def
    /Yordonnee Xcercle C1 mul neg Ycercle S2 S1 mul mul add YO' add
    def
    /Zcote Ycercle C2 mul neg ZO' add def
    CalcCoordinates ]
    } for
    ] def
 TableauxPoints 0 get aload pop moveto
 0 1 359 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
 end
}% fin du code ps
\showpointsfalse
\end@ClosedObj
}}
%
%
\def\FrameThreeD{\pst@object{FrameThreeD}}
\def\FrameThreeD@i{\@ifnextchar[{\FrameThreeD@do}{\FrameThreeD@do[]}}
\def\FrameThreeD@do[#1](#2,#3)(#4,#5){{%
% (#2,#3) d'un sommet
% (#4,#5) du sommet opposé
% rectangle ABCD
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
/XA #2 def
/YA #3 def
/XC #4 def
/YC #5 def
% on en déduit les autres sommets
/XB XC def
/YB YA def
/XD XA def
/YD YC def
\variablesTroisD
/XO' \psk@TroisD@Xorigine\space def
/YO' \psk@TroisD@Yorigine\space def
/ZO' \psk@TroisD@Zorigine\space def
tx@3DDict begin
reduction reduction scale
newpath
    /Xframe XA def
    /Yframe YA def
    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add XO' add
    def
    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add YO' add
    def
    /Zcote Yframe C2 mul neg ZO' add def
    CalcCoordinates
     moveto
    /Xframe XB def
    /Yframe YB def
    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add XO' add
    def
    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add YO' add
    def
    /Zcote Yframe C2 mul neg ZO' add def
    CalcCoordinates
    lineto
    /Xframe XC def
    /Yframe YC def
    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add XO' add
    def
    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add YO' add
    def
    /Zcote Yframe C2 mul neg ZO' add def
    CalcCoordinates
    lineto
    /Xframe XD def
    /Yframe YD def
    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add XO' add
    def
    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add YO' add
    def
    /Zcote Yframe C2 mul neg ZO' add def
    CalcCoordinates
    lineto
    /Xframe XA def
    /Yframe YA def
    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add XO' add
    def
    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add YO' add
    def
    /Zcote Yframe C2 mul neg ZO' add def
    CalcCoordinates
    lineto
closepath
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}% % fin de la commande PSTricks
%
%
\def\QuadrillageThreeD{\pst@object{QuadrillageThreeD}}
\def\QuadrillageThreeD@i{\@ifnextchar[{\QuadrillageThreeD@do}{\QuadrillageThreeD@do[]}}
\def\QuadrillageThreeD@do[#1]{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@OpenObj
\addto@pscode{%
\variablesTroisD
/XO' \psk@TroisD@Xorigine\space def
/YO' \psk@TroisD@Yorigine\space def
/ZO' \psk@TroisD@Zorigine\space def
/Xmax \psk@TroisD@Xmax\space def
/Ymax \psk@TroisD@Ymax\space def
/Xmin \psk@TroisD@Xmin\space def
/Ymin \psk@TroisD@Ymin\space def
/pas \psk@TroisD@pas\space def
/grille \psk@TroisD@grille\space def
tx@3DDict begin
reduction reduction scale
Ymin grille Ymax {% balayage suivant Oy
    /Ygrille exch def
/TableauxPoints [
    Xmin pas Xmax { % balayage suivant Ox
    /Xgrille exch def
    /Xabscisse Xgrille S1 mul Ygrille S2 C1 mul mul add XO' add
    def
    /Yordonnee Xgrille C1 mul neg Ygrille S2 S1 mul mul add YO' add
    def
    /Zcote Ygrille C2 mul neg ZO' add def
    formulesTroisD
        [
         Xi 28.45 mul Yi 28.45 mul %
        ]
        } for
    ] def
 TableauxPoints 0 get aload pop moveto
 0 1 Xmax Xmin sub pas div {
    /compteur exch def
    TableauxPoints compteur get aload pop
   lineto } for
% stroke
    } for
%
Xmin grille Xmax {% balayage suivant Ox
    /Xgrille exch def
/TableauxPoints [
    Ymin pas Ymax { % balayage suivant Ox
    /Ygrille exch def
    /Xabscisse Xgrille S1 mul Ygrille S2 C1 mul mul add XO' add
    def
    /Yordonnee Xgrille C1 mul neg Ygrille S2 S1 mul mul add YO' add
    def
    /Zcote Ygrille C2 mul neg ZO' add def
    formulesTroisD
        [
         Xi 28.45 mul Yi 28.45 mul %
        ]
        } for
    ] def
 TableauxPoints 0 get aload pop moveto
  0 1 Ymax Ymin sub pas div {
    /compteur exch def
    TableauxPoints compteur get aload pop
   lineto } for
  \pst@number\pslinewidth SLW
  \pst@usecolor\pslinecolor
  \@nameuse{psls@\pslinestyle}
% stroke
    } for
% fin du tracé
end
 }% fin du code ps
 \end@OpenObj
 }}% % fin de la commande PSTricks
%
%
% 11 novembre
\def\DemiSphereThreeD{\pst@object{DemiSphereThreeD}}
\def\DemiSphereThreeD@i{\@ifnextchar[{\DemiSphereThreeD@do}{\DemiSphereThreeD@do[]}}
\def\DemiSphereThreeD@do[#1]#2{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
    /increment 10 def
tx@3DDict begin
/condition {PSfacette 0 le} def
/departPhi 0 def
MaillageSphere
% centre de la base inférieure après transformations
    /CxFaceInf CX def
    /CyFaceInf CY def
    /CzFaceInf CZ def
% correction 16 novembre 2002
%    /Xpoint CxFaceInf def
%    /Ypoint CyFaceInf def
%    /Zpoint CzFaceInf def
    /Xpoint 0 def
    /Ypoint 0 def
    /Zpoint 0 def
% fin correction 16/11/2002
CalculsPointsAfterTransformations
    /CxBaseInf Xabscisse def
    /CyBaseInf Yordonnee def
    /CzBaseInf Zcote def
    /RXvueInf CxBaseInf XpointVue sub def
    /RYvueInf CyBaseInf YpointVue sub def
    /RZvueInf CzBaseInf ZpointVue sub def
% Sommet de la sphère
    /Xpoint 0 def
    /Ypoint 0 def
    /Zpoint Rsphere def
CalculsPointsAfterTransformations
    /XsommetSphere Xabscisse def
    /YsommetSphere Yordonnee def
    /ZsommetSphere Zcote def
% Normale extérieure à la base inférieure
    /nXBaseInf CxFaceInf XsommetSphere sub def
    /nYBaseInf CyFaceInf YsommetSphere sub def
    /nZBaseInf CzFaceInf ZsommetSphere sub def
% Visibilité de la base inférieure
    /PSbaseSphere nXBaseInf RXvueInf mul
                  nYBaseInf RYvueInf mul add
                  nZBaseInf RZvueInf mul add def
PSbaseSphere 0 le {
/TableauxPoints [
0 1 359 {% on décrit le cercle
    /theta exch def [
    /Xpoint Rsphere theta cos mul def
    /Ypoint Rsphere theta sin mul def
    /Zpoint 0 def
CalculsPointsAfterTransformations
    CalcCoordinates ]
    } for
    ] def
gsave
newpath
 TableauxPoints 0 get aload pop moveto
0 1 359 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
0.7 setgray
closepath
fill
grestore
 } if
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}% % fin de la commande PSTricks
%
%
\def\SphereCreuse{\pst@object{SphereCreuse}}
\def\SphereCreuse@i{\@ifnextchar[{\SphereCreuse@do}{\SphereCreuse@do[]}}
\def\SphereCreuse@do[#1]#2{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
    /increment 10 def
tx@3DDict begin
/SphereInside {
/condition {PSfacette 0 ge} def
/departPhi 0 def
MaillageSphere
} def
%
% centre de la base inférieure après transformations
    /CxFaceInf CX def
    /CyFaceInf CY def
    /CzFaceInf CZ def
    /Xpoint CxFaceInf def
    /Ypoint CyFaceInf def
    /Zpoint CzFaceInf def
CalculsPointsAfterTransformations
    /CxBaseInf Xabscisse def
    /CyBaseInf Yordonnee def
    /CzBaseInf Zcote def
    /RXvueInf CxBaseInf XpointVue sub def
    /RYvueInf CyBaseInf YpointVue sub def
    /RZvueInf CzBaseInf ZpointVue sub def
% Sommet de la sphère
    /Xpoint 0 def
    /Ypoint 0 def
    /Zpoint Rsphere def
CalculsPointsAfterTransformations
    /XsommetSphere Xabscisse def
    /YsommetSphere Yordonnee def
    /ZsommetSphere Zcote def
% Normale extérieure à la base inférieure
    /nXBaseInf CxFaceInf XsommetSphere sub def
    /nYBaseInf CyFaceInf YsommetSphere sub def
    /nZBaseInf CzFaceInf ZsommetSphere sub def
% Visibilité de la base inférieure
    /PSbaseSphere nXBaseInf RXvueInf mul
                  nYBaseInf RYvueInf mul add
                  nZBaseInf RZvueInf mul add def
/base {
/TableauxPoints [
0 1 359 {% on décrit le cercle
    /theta exch def [
    /Xpoint Rsphere theta cos mul def
    /Ypoint Rsphere theta sin mul def
    /Zpoint 0 def
CalculsPointsAfterTransformations
    CalcCoordinates ]
    } for
    ] def
% gsave
newpath
 TableauxPoints 0 get aload pop moveto
0 1 359 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
0.7 setgray
closepath
% stroke
%grestore
} def
PSbaseSphere 0 le {
base
clip
SphereInside
 } { 0 0 0.01 0 360 arc } ifelse
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}% % fin de la commande PSTricks
%
% 30 novembre
\def\PortionSphere{\pst@object{PortionSphere}}
\def\PortionSphere@i{\@ifnextchar[{\PortionSphere@do}{\PortionSphere@do[]}}
\def\PortionSphere@do[#1]#2{{%
% #2 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
\variablesTroisD
reduction reduction scale
    /Rsphere #2 def
    /increment 1 def
tx@3DDict begin
    /Xpoint Rsphere psTHETA dTHETA neg add cos mul psPHI dPHI sub cos mul def
    /Ypoint Rsphere psTHETA dTHETA neg add sin mul psPHI dPHI sub cos mul def
    /Zpoint Rsphere psPHI dPHI sub sin mul def
CalculsPointsAfterTransformations
CalcCoordinates
newpath
     moveto
psTHETA dTHETA sub 1 psTHETA dTHETA add {
    /Theta exch def
    /Xpoint Rsphere Theta cos psPHI dPHI sub cos mul mul def
    /Ypoint Rsphere Theta sin psPHI dPHI sub cos mul mul def
    /Zpoint Rsphere psPHI dPHI sub sin mul def
    CalculsPointsAfterTransformations
    CalcCoordinates
     lineto
     } for
psPHI dPHI sub 1 psPHI dPHI add {
    /Phi exch def
    /Xpoint Rsphere psTHETA dTHETA add cos Phi cos mul mul def
    /Ypoint Rsphere psTHETA dTHETA add sin Phi cos mul mul def
    /Zpoint Rsphere Phi sin mul def
    CalculsPointsAfterTransformations
    CalcCoordinates
     lineto
     } for
psTHETA dTHETA add -1 psTHETA dTHETA sub {
    /Theta exch def
    /Xpoint Rsphere Theta cos psPHI dPHI add cos mul mul def
    /Ypoint Rsphere Theta sin psPHI dPHI add cos mul mul def
    /Zpoint Rsphere psPHI dPHI add sin mul def
    CalculsPointsAfterTransformations
    CalcCoordinates
     lineto
     } for
psPHI dPHI add -1 psPHI dPHI sub {
    /Phi exch def
    /Xpoint Rsphere psTHETA dTHETA sub cos Phi cos mul mul def
    /Ypoint Rsphere psTHETA dTHETA sub sin Phi cos mul mul def
    /Zpoint Rsphere Phi sin mul def
    CalculsPointsAfterTransformations
    CalcCoordinates
     lineto
     } for
closepath
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}% % fin de la commande PSTricks
%
%% END: pst-3DNew.tex

